Model Cascading: Towards Jointly Improving Efficiency and Accuracy of NLP Systems

Do all instances need inference through the big models for a correct prediction? Perhaps not; some instances are easy and can be answered correctly by even small capacity models. This provides opportunities for improving the computational efficiency of systems. In this work, we present an explorative study on 'model cascading', a simple technique that utilizes a collection of models of varying capacities to accurately yet efficiently output predictions. Through comprehensive experiments in multiple task settings that differ in the number of models available for cascading (K value), we show that cascading improves both the computational efficiency and the prediction accuracy. For instance, in K=3 setting, cascading saves up to 88.93% computation cost and consistently achieves superior prediction accuracy with an improvement of up to 2.18%. We also study the impact of introducing additional models in the cascade and show that it further increases the efficiency improvements. Finally, we hope that our work will facilitate development of efficient NLP systems making their widespread adoption in real-world applications possible.

==> Tables/analysis_K_2.tex <==
\begin{table*}[]
% \small
\resizebox{\textwidth}{!}{%
\begin{tabular}{l|ll|ll|ll|ll|ll|ll|ll|ll|ll|ll}
% \begin{tabular}{ll|lllllllllll}
\toprule
% \multicolumn{1}{c}{\multirow{1}{*}{\textbf{Model}}} &
%   \multicolumn{1}{c}{\multirow{1}{*}{\textbf{Metric}}}  &
\multicolumn{1}{c}{\textbf{}} &
  \multicolumn{2}{c}{\textbf{MNLI}} &
  \multicolumn{2}{c}{\textbf{QNLI}} &
  \multicolumn{2}{c}{\textbf{QQP}} &
  \multicolumn{2}{c}{\textbf{SST2}} &
  \multicolumn{2}{c}{\textbf{COLA}} &
  \multicolumn{2}{c}{\textbf{CB}} &
  \multicolumn{2}{c}{\textbf{DNLI}} &
  \multicolumn{2}{c}{\textbf{MRPC}} &
  \multicolumn{2}{c}{\textbf{PAWS}} &
  \multicolumn{2}{c}{\textbf{SNLI}} \\

 &
M1 & M2 &
M1 & M2 &
M1 & M2 &
M1 & M2 &
M1 & M2 &
M1 & M2 &
M1 & M2 &
M1 & M2 &
M1 & M2 &
M1 & M2 \\



  

\midrule

    % MaxProb & 
    % 81.7567 &  84.9926 &  90.0535 &  89.8323 &  79.6548 &  80.8606 &  85.471 &  81.9074 &  91.9684 &  89.954 \\
    
    \textbf{\%} &
    11.11 & 11.11 &
    11.11 & 11.11 &
    11.11 & 11.11 &
    11.11 & 11.11 &
    11.11 & 11.11 &
    11.11 & 11.11 &
    11.11 & 11.11 &
    11.11 & 11.11 &
    11.11 & 11.11 &
    11.11 & 11.11 \\
    
    \textbf{M1} &
    11.11 & 11.11 &
    11.11 & 11.11 &
    11.11 & 11.11 &
    11.11 & 11.11 &
    11.11 & 11.11 &
    11.11 & 11.11 &
    11.11 & 11.11 &
    11.11 & 11.11 &
    11.11 & 11.11 &
    11.11 & 11.11 \\
    
    \textbf{M2} &
    11.11 & 11.11 &
    11.11 & 11.11 &
    11.11 & 11.11 &
    11.11 & 11.11 &
    11.11 & 11.11 &
    11.11 & 11.11 &
    11.11 & 11.11 &
    11.11 & 11.11 &
    11.11 & 11.11 &
    11.11 & 11.11 \\
    
    

\bottomrule
\end{tabular}
}
\caption{Analysis K=2}
\label{tab:analysis_K_2}

\end{table*}


==> Tables/perf_K_2.tex <==
\begin{table*}[]
\small
\resizebox{\textwidth}{!}{%
\begin{tabular}{llllllllllll}
% \begin{tabular}{ll|lllllllllll}
\toprule
% \multicolumn{1}{c}{\multirow{1}{*}{\textbf{Model}}} &
%   \multicolumn{1}{c}{\multirow{1}{*}{\textbf{Metric}}}  &
%   \multicolumn{1}{c}{\textbf{MNLI}} &
%   \multicolumn{1}{c}{\textbf{MNLI}} &
%   \multicolumn{1}{c}{\textbf{MNLI}} &
%   \multicolumn{1}{c}{\textbf{MNLI}} &
%   \multicolumn{1}{c}{\textbf{MNLI}} &
%   \multicolumn{1}{c}{\textbf{MNLI}} &
%   \multicolumn{1}{c}{\textbf{MNLI}} &
%   \multicolumn{1}{c}{\textbf{MNLI}} &
%   \multicolumn{1}{c}{\textbf{MNLI}} &
%   \multicolumn{1}{c}{\textbf{MNLI}}

\textbf{Method} & \textbf{Metric} &
\textbf{MNLI} &  \textbf{QNLI} &  \textbf{QQP} &  \textbf{SST2} &  \textbf{COLA} &  \textbf{CB} &  \textbf{DNLI} &  \textbf{MRPC} &  \textbf{PAWS} &  \textbf{SNLI} \\ 
  

\midrule
\multirow{2}{*}{Base}
    & Cost & 
    10.1928 &  12.7408 &  8.4941 &  6.7954 &  4.2473 &  23.3576 &  10.1928 &  12.7408 &  12.7408 &  10.1928 \\ 
    
    & Acc & 
    82.53 &  86.02 &  89.99 &  90.14 &  81.29 &  82.14 &  85.93 &  83.1 &  92.21 &  90.01  \\
    
    
    
    
    

% \multirow{2}{*}{Med}
%     & Acc & 
%     80.32 &  83.43 &  89.51 &  88.88 &  77.64 &  75 &  85.18 &  81.03 &  91.43 &  89.13 \\ 
    
%     & Cost & 
%     3.0202 &  3.7751 &  2.5168 &  2.0135 &  1.2586 &  6.9209 &  3.0202 &  3.7751 &  3.7751 &  3.0202 \\ 
    
    

    
\midrule
\multirow{2}{*}{Cascading}
    & Cost@base acc & 
    5.2627 &  7.9559 &  2.82 &  2.9564 &  3.7083 &  11.9261 &  13.213 &  8.4936 &  5.0565 &  3.9753 \\
    
    & Acc@base cost & 
    82.89 &  86.23 &  90.39 &  90.48 &  81.38 &  82.14 &  85.93 &  83.47 &  92.47 &  90.4 \\ 
    
    % & AUC & 
    % 81.7567 &  84.9926 &  90.0535 &  89.8323 &  79.6548 &  80.8606 &  85.471 &  81.9074 &  91.9684 &  89.954 \\ 
    
% \midrule

% \multirow{3}{*}{HmSH}
%     & Cost@base acc & 90.90 & 90.90 & 90.90 & 90.90 & 90.90 & 90.90 & 90.90 & 90.90 & 90.90 & 90.90 \\
    
%     & Acc@base acc & 90.90 & 90.90 & 90.90 & 90.90 & 90.90 & 90.90 & 90.90 & 90.90 & 90.90 & 90.90 \\
    
%     & AUC & 90.90 & 90.90 & 90.90 & 90.90 & 90.90 & 90.90 & 90.90 & 90.90 & 90.90 & 90.90 \\
    

\bottomrule
\end{tabular}
}

\caption{K=2 using Bert-medium and bert-base}
\label{tab:perf_K_2}

\end{table*}


==> Tables/random_approach_illustration.tex <==
\begin{table}[t]
    \centering
    % \small
    \begin{tabular}{@{}c|cc|c@{}}
        \toprule
        \textbf{\#Scenario} &  \textbf{$M_1$} & \textbf{$M_2$} & \textbf{N*Cost}\\
        \midrule
        1 & N & 0 & $c_1*(N) + c_2*0$\\
        2 & N-1 & 1 & $c_1*(N-1) + c_2*1$\\
        3 & N-2 & 2 & $c_1*(N-2) + c_2*2$\\
        ... & ... & ... & ...\\
        N & 1 & N-1 & $c_1*1 + c_2*(N-1)$\\
        N+1 & 0 & N  & $c_1*0 + c_2*(N)$\\
        
        
    \bottomrule
    \end{tabular}
    \caption{Illustrating accuracy-cost pairs collection procedure for `Random' cascading method in $K=2$ setting. We divide the evaluation dataset (having $N$ instances) between models $M_1$ and $M_2$ in each possible proportion and compute accuracy, cost value for each scenario. $c_1$ and $c_2$ correspond to the computation cost of $M_1$ and $M_2$ respectively.}
    
    % enumerating all possible combinations of dividing an evaluation dataset having $N$ instances between the two models $M_1$ and $M_2$. In `Random' cascading method, we randomly divide the instances for each combination and compute the system's accuracy and computation cost. 
    \label{tab:random_approach_illustration}
\end{table}
